Deep learning based spatial aliasing reduction in beamforming for audio capture

Spatial aliasing affects spaced microphone arrays, causing directional ambiguity above certain frequencies, degrading spatial and spectral accuracy of beamformers. Given the limitations of conventional signal processing and the scarcity of deep learning approaches to spatial aliasing mitigation, we propose a novel approach using a U-Net architecture to predict a signal-dependent de-aliasing filter, which reduces aliasing in conventional beamforming for spatial capture. Two types of multichannel filters are considered, one which treats the channels independently and a second one that models cross-channel dependencies. The proposed approach is evaluated in two common spatial capture scenarios: stereo and first-order Ambisonics. The results indicate a very significant improvement, both objective and perceptual, with respect to conventional beamforming. This work shows the potential of deep learning to reduce aliasing in beamforming, leading to improvements in multi-microphone setups.

==> Section_5/Subsection_1.tex <==
\subsection{Cardioid pair de-aliasing setup}
The first experiment considers the case of two opposite-facing cardioid beams, a common setup for obtaining stereo signals from a pair of closely spaced omnidirectional microphones \cite{faller2010conversion}.
Given the raw mixture signals, the virtual microphone signals are obtained by calculating the pressure gradient for the X-axis pair of the aforementioned 4-channel microphone array, which results in quasi frequency-independent characteristics.
In this experimental setup, we use an identity decoder, so the spatial responses of the virtual microphone signals are explicitly optimized for, as discussed in Section \ref{sec:section_3}.
To obtain suitable alias-free target signals, we follow the procedure described in Section \ref{sec:section_4}, with \shpCoe{}=0.5 in equation \eqref{eq:polar_patterns}.
In this experiment, \numVrtMic{}=2 and \dirNum{}=2. 

\begin{comment}
\begin{table}[]
\caption{C-Si-SNR values for the experiment with cardioid pair de-aliasing, given in dB. The numbers in parentheses denote improvement.}
\label{tab:first_experiment}
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{filter type / aliasing type}} &
  \textbf{fixed} &
  \textbf{varying} \\ \hline
diagonal &
  \begin{tabular}[c]{@{}c@{}}30.26\\ (19.54)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}15.42\\ (7.59)\end{tabular} \\ \hline
full &
  \begin{tabular}[c]{@{}c@{}}27.26\\ (16.57)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}20.19\\ (12.36)\end{tabular} \\ \hline
\end{tabular}
\end{table}
\end{comment}


==> Section_5/Subsection_2.tex <==
\subsection{2D Ambisonics de-aliasing setup}

The second experiment aims at de-aliasing horizontal FOA obtained from the array of four microphones. Pressure gradient is applied to the pairs along the x and y axes to obtain X and Y figure-of-eight signals respectively, while the omnidirectional W is obtained by averaging the four signals. $\decMat$ is an in-phase decoder to four cardioids along the front, back, left and right directions.
In this experiment, \numVrtMic{}=3 and \dirNum{}=4.

\begin{comment}
\begin{table}[]
\caption{C-Si-SNR values for the experiment with 2D Ambisonics de-aliasing, given in dB. The numbers in parentheses denote improvement.}
\label{tab:second_experiment}
\begin{tabular}{|l|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{filter type / aliasing type}} &
  \textbf{fixed} &
  \textbf{varying} \\ \hline
diagonal &
  \begin{tabular}[c]{@{}c@{}}29.31\\ (11.26)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}19.68\\ (7.75)\end{tabular} \\ \hline
full &
  \begin{tabular}[c]{@{}c@{}}28.89\\ (10.21)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}19.49\\ (7.56)\end{tabular} \\ \hline
\end{tabular}
\end{table}
\end{comment}
\begin{comment}
    \begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{Section_5/ABAB2Ambisonics2DUNet_channel=0_1.pdf}
    \caption{Spatial responses of the decoded signals }
    \label{fig:first_experiment}
\end{figure}
\end{comment}


